Towards Long-Tailed 3D Detection

Contemporary autonomous vehicle (AV) benchmarks have advanced techniques for training 3D detectors, particularly on large-scale lidar data. Surprisingly, although semantic class labels naturally follow a long-tailed distribution, contemporary benchmarks focus on only a few common classes (e.g., pedestrian and car) and neglect many rare classes in-the-tail (e.g., debris and stroller). However, AVs must still detect rare classes to ensure safe operation. Moreover, semantic classes are often organized within a hierarchy, e.g., tail classes such as child and construction-worker are arguably subclasses of pedestrian. However, such hierarchical relationships are often ignored, which may lead to misleading estimates of performance and missed opportunities for algorithmic innovation. We address these challenges by formally studying the problem of Long-Tailed 3D Detection (LT3D), which evaluates on all classes, including those in-the-tail. We evaluate and innovate upon popular 3D detection codebases, such as CenterPoint and PointPillars, adapting them for LT3D. We develop hierarchical losses that promote feature sharing across common-vs-rare classes, as well as improved detection metrics that award partial credit to "reasonable" mistakes respecting the hierarchy (e.g., mistaking a child for an adult). Finally, we point out that fine-grained tail class accuracy is particularly improved via multimodal fusion of RGB images with LiDAR; simply put, small fine-grained classes are challenging to identify from sparse (lidar) geometry alone, suggesting that multimodal cues are crucial to long-tailed 3D detection. Our modifications improve accuracy by 5% AP on average for all classes, and dramatically improve AP for rare classes (e.g., stroller AP improves from 3.6 to 31.6)! Our code is available at https://github.com/neeharperi/LT3D

==> figures/backup.tex <==
{
\setlength{\tabcolsep}{0.75em} % for the horizontal padding
\begin{table}[t]
\small
% \scriptsize
\centering
\caption{\small 
{\bf Benchmarking detectors for \problem} leads to several salient conclusiosn. 
Firstly, training with the semantic hierarchy improves all methods for \problem, e.g., improving PointPillars and CBGS by 1 AP and  CenterPoint by 3 AP {\tt All} classes. It seems to have a bigger impact on the heatmap-based detector head than the standard anchor-based detector heads. It also slightly helps multimodal detectors (within 1 AP for MVP and TransFusion).
Secondly, multimodal filtering yields 4$\sim$11 AP improvement on {\tt Medium} and {\tt Few} classes! This is surprising given that FCOS3D is a less powerful 3D detector on its own. Interestingly, it also improves multimodal detectors (3.4  and 1.6 AP improvement for MVP and TransFusion on {\tt All} classes), demonstrating the importance of using RGB to improve \problem\ with better recognition.
Thirdly, perhaps surprisingly, the best model is to use LiDAR-only detector CenterPoint and RGB-only detector FCOS3D, surpassing multimodal detectors MVP and TransFusion.
% seemingly suggesting that filtering works the best with more aggressive false positives.
Lastly, data augmentation schedule does not necessarily improve \problem \ performance, demonstrating the challenge of 3D detection in the long-tail.
%\deva{Minor point; I'd move NDS to supplement. I don't really trust the metric and it somewhat deflates the story.}
 }
\begin{tabular}{l c c c c c c c c c c c}
\toprule
\multirow{2}{*}{Method} & \multirow{2}{*}{Multimodal} & \multicolumn{2}{c}{\tt Many} & \multicolumn{2}{c}{\texttt{Medium}} & \multicolumn{2}{c}{\texttt{Few}} & \multicolumn{2}{c}{\tt All} \\ 
% \cline{4-11} 
\cmidrule(lr){3-4}
\cmidrule(lr){5-6}
\cmidrule(lr){7-8}
\cmidrule(lr){9-10}
                                                   &            & {mAP}     & {NDS}   & {mAP}  &    {NDS}   & {mAP}  &    {NDS}   & {mAP}   & {NDS}  \\
\midrule
\multirow{1}{*}{FCOS3D}                            &           &  39.0         &   47.2     & 23.3      &      34.8     &   2.9     &      15.7    &   20.9     &    31.9   \\

\midrule 
\midrule

\multirow{1}{*}{PointPillars}                      &            &  64.2         &   64.5     & 28.4      &      41.5     &   3.4     &      22.1    &   30.0     &    41.4   \\ 
\multirow{1}{*}{$\indent$ + Hierarchy}             &           &  66.4         &   65.8     & 30.4      &      43.2     &   2.9     &      23.0    &   31.2     &    42.7   \\
\multirow{1}{*}{$\indent$ w/ Data Aug.}            &            &  54.4         &   55.6     & 24.2      &      38.2     &   1.8     &      14.7    &   25.1     &    35.2   \\ 
\multirow{1}{*}{$\indent$ w/ Filtering}            & \checkmark  &  66.2         &   65.7     & 41.0      &      48.7     &   4.4     &      18.9    &   35.8     &    43.5   \\

\midrule
\multirow{1}{*}{CBGS}                             &             &  47.2         &   52.3     & 10.4      &    29.7     &   0.1     &      15.4    &   17.2     &    31.2   \\
\multirow{1}{*}{$\indent$ + Hierarchy}            &             &  49.5         &   53.3     & 11.1      &     29.6     &   0.1     &      16.7    &   18.1     &    31.9   \\
\multirow{1}{*}{$\indent$ w/ Data Aug.}           &             &  49.9         &   53.7     & 17.1      &      32.7     &   0.1     &      14.8    &   20.6     &    32.5   \\ 
\multirow{1}{*}{$\indent$ w/ Filtering}           &  \checkmark         &  48.0         &   52.7     & 20.3      &      34.4     &   0.1     &      11.9    &   21.5     &    32.0   \\

\midrule
\multirow{1}{*}{CenterPoint}                       &            &  73.7         &   71.8     & 41.3      &      51.2     &   3.0     &      26.8    &   37.5     &    48.8   \\ 
\multirow{1}{*}{$\indent$ + Hierarchy}          &               &  77.1         &   73.5     & 45.1      &      52.5     &   4.3     &      25.4    &   40.4     &    49.3   \\
\multirow{1}{*}{$\indent$ w/ Data Aug.}         &               &  73.8         &   70.7     & 44.5      &      51.2     &   7.4     &      25.6    &   40.3     &    48.1   \\ 
\multirow{1}{*}{$\indent$ w/ Filtering}         &   \checkmark            &  77.1         &   73.5     & 49.0      &      54.9     &   9.4     &      23.5    &   43.6     &    49.6   \\ 

\midrule
\midrule
\multirow{1}{*}{MVP}                             &  \checkmark            &  65.6         &   63.9     & 31.6      &      40.1     &   1.5     &      16.6    &   31.0     &    38.9   \\ 
\multirow{1}{*}{$\indent$ + Hierarchy}           &  \checkmark            &  67.0         &   64.4     & 33.0      &      39.9     &   0.1     &      15.1    &   31.6     &    38.4   \\
\multirow{1}{*}{$\indent$ w/ Data Aug.}          &  \checkmark            &  65.9         &   63.3     & 35.8      &      41.4     &   0.1     &      21.2    &   32.5     &    40.8   \\ 
\multirow{1}{*}{$\indent$ w/ Filtering}          &   \checkmark         &  67.1         &   64.3     & 39.2      &      43.3     &   1.6     &      14.4   &  34.4     &   39.5  \\ 

\midrule
\multirow{1}{*}{TransFusion}                   &                  &  68.5         &   73.0     & 42.8      &      53.4     &   8.4     &      31.3    &   38.5     &    51.5   \\ 
\multirow{1}{*}{$\indent$ + Camera}              &  \checkmark      &  73.9         &   75.5     & 41.2      &      52.4     &   9.8     &      34.6    &   39.8     &    52.9   \\
\multirow{1}{*}{$\indent$ w/ Data Aug.}          &  \checkmark      &  73.4         &   75.0     & 40.9      &      52.1     &   8.2     &      34.4    &   39.0     &    52.5   \\ 
\multirow{1}{*}{$\indent$ w/ Filtering}          &  \checkmark      &  73.9         &   75.5     & 42.5      &      53.4     &   9.1     &      31.5    &  40.1     &    52.3   \\ 
\bottomrule
\end{tabular}
\label{tab:lt3d}
\vspace{-5mm}
\end{table}
}
